Gender Segregation: Analysis across Sectoral-Dominance in the UK Labour Market

This paper aims to evaluate how changing patterns of sectoral gender segregation play a role in accounting for women's employment contracts and wages in the UK between 2005 and 2020. We then study wage differentials in gender-specific dominated sectors. We found that the propensity of women to be distributed differently across sectors is a major factor contributing to explaining the differences in wages and contract opportunities. Hence, the disproportion of women in female-dominated sectors implies contractual features and lower wages typical of that sector, on average, for all workers. This difference is primarily explained by "persistent discriminatory constraints", while human capital-related characteristics play a minor role. However, wage differentials would shrink if workers had the same potential and residual wages as men in male-dominated sectors. Moreover, this does not happen at the top of the wage distribution, where wage differentials among women working in female-dominated sectors are always more pronounced than those of men.

==> figures.tex <==
\section*{Figures}
\begin{figure}[h!]
	 \caption{Distribution of gender sectoral segregation index, by sectoral dominance}\label{fig:kdensity_dom}
  \centering
	{\includegraphics[scale=.90]{figs/kdensity_dominance.pdf}}
\end{figure}

\begin{figure}[h!]
	 \caption{Distribution of gender sectoral segregation index, by sectoral dominance and degree of segregation}\label{fig:kdensity_hl}
  \centering
	{\includegraphics[scale=.9]{figs/kdensity_hl_rank.pdf}}
\end{figure}

%%shift
\begin{figure}
	 \caption{Shift-share decomposition of employment, by female sample}\label{fig:shift_share_all}
  \centering
		\includegraphics[scale=.85]{figs/line_shift_share_fml_pres.pdf}
	 \begin{minipage}{.85\linewidth}
	\vspace{3mm}
	\footnotesize
	\emph{Note:  The graph shows the difference in employment in the comparison year with respect to the base year (i.e., the fiscal year 2005). The overall change in employment is shown in solid line and  its decomposition into the \emph{between} and \emph{within} components respectively, with dashed and dotted lines. The cross marks the components for  female-dominated sectors and the circle  the components  for male sectors. The \emph{between} component (BTW) captures the change due to changes in the sectoral structure of the economy;  the \emph{within} component (WTHN) reflects changes in female composition within sectors.}
	\end{minipage}
\end{figure}

%%%%%%%%%PSM
\begin{figure}[tb!] 
	 \caption{Covariate imbalance test, single components}\label{fig:balance}
  \centering
	\subfloat[Pooled sample]{\includegraphics[scale=.55]{figs/psm_balance_check.pdf}}\\
	\subfloat[Male sample]{\includegraphics[scale=.55]{figs/psm_balance_check2_gender0.pdf}}\\
	\subfloat[Female sample]{\includegraphics[scale=.55]{figs/psm_balance_check2_gender1.pdf}}\\
	\begin{minipage}{.75\linewidth}
	\vspace{3mm}
	\footnotesize
	\emph{Note: The included covariates are balanced if the standardised bias after matching is within $\pm 5\%$ \citep{rosenbaum1985}. If the condition is satisfied, the matching method successfully builds a valid control group.}
	\end{minipage}
\end{figure}	

%%%KBO DECOMPOSITION
\begin{figure}[th!] 
\vspace{8mm}
	 \caption{KBO decomposition, by gender sectoral dominance}\label{fig:oaxaca_dom}
  \centering
	\includegraphics[scale=1]{figs/bo_mf_dom2.pdf}\\
	 \begin{minipage}{.9\linewidth}
	\vspace{3mm}
	\footnotesize
	\emph{\textsc{Estimation note}: Both models for women and men are estimated using the Mincerian regression equation (with OLS). The degree of gender segregation is not included because it is highly correlated with the grouping variable of gender sectoral dominance. The shaded areas are the 95\% confidence intervals.}
	\end{minipage}
\end{figure}	

\begin{figure}[tb!]
	 \caption{CDFs of predicted wages, by gender and sectoral dominance}\label{fig:cdf_yhat}
  \centering
	{\includegraphics[scale=1.05]{figs/cdf_comparison_yhat.pdf}}\\
		 \begin{minipage}{.85\linewidth}
	\vspace{3mm}
	\footnotesize
	\emph{Note: The solid line is for men working in male-dominated sectors, the short-dashed line is for women employed in male-dominated sectors, the long-dash line is for men in female-dominated sectors, and the dash-dot line is for women in female-dominated sectors. Left: Predicted wages are calculated after estimating the coefficients of the Mincerian wage regression, reported in Table~\ref{tab:mincer_regs}. Right: predicted wages are calculates using  the estimated coefficients from the  Mincerian regression of men working in male-dominated sectors. Predicted wages in the counterfactual exercise are precise measure of individual earnings potential  \citep{gould2016,borjas2019}.}
	\end{minipage}
\end{figure}

\begin{figure}[tb!]
	 \caption{CDFs of residual wages, by gender and sectoral dominance}\label{fig:cdf_uhat}
  \centering
	{\includegraphics[scale=1.05]{figs/cdf_comparison_uhat.pdf}}\\
		 \begin{minipage}{.85\linewidth}
	\vspace{3mm}
	\footnotesize
	\emph{Note: The solid line is for men working in male-dominated sectors, the short-dashed line is for women employed in male-dominated sectors, the long-dash line is for men in female-dominated sectors, and the dash-dot line is for women in female-dominated sectors. Left: Residual wages are calculated after estimating the coefficients of the Mincerian wage regression, reported in Table~\ref{tab:mincer_regs}. Right: Residual wages are calculates using  the estimated coefficients from the  Mincerian regression of men working in male-dominated sectors. Residuals from a Mincerian regression calculated in this way capture the part of earnings that is uncorrelated to observed skills \citep{parey2017}.}
	\end{minipage}
\end{figure}

==> tables.tex <==
\section*{Tables}

\input{tabs/tab_share_fml.tex}
\input{tabs/tab_sic_soc_ml.tex}
\input{tabs/tab_sic_soc_fml.tex}

\input{tabs/sum_stats.tex}
\input{tabs/tab_pt.tex}
\input{tabs/probit_inlf.tex}	
\input{tabs/sectors2.tex}

\input{tabs/psm_results_together.tex}	
\input{tabs/wage_regs.tex}	
\input{tabs/ksmirnov.tex}


